Do Vision-Language Models Really Understand Visual Language?

Visual language is a system of communication that conveys information through symbols, shapes, and spatial arrangements. Diagrams are a typical example of a visual language depicting complex concepts and their relationships in the form of an image. The symbolic nature of diagrams presents significant challenges for building models capable of understanding them. Recent studies suggest that Large Vision-Language Models (LVLMs) can even tackle complex reasoning tasks involving diagrams. In this paper, we investigate this phenomenon by developing a comprehensive test suite to evaluate the diagram comprehension capability of LVLMs. Our test suite uses a variety of questions focused on concept entities and their relationships over a set of synthetic as well as real diagrams across domains to evaluate the recognition and reasoning abilities of models. Our evaluation of LVLMs shows that while they can accurately identify and reason about entities, their ability to understand relationships is notably limited. Further testing reveals that the decent performance on diagram understanding largely stems from leveraging their background knowledge as shortcuts to identify and reason about the relational information. Thus, we conclude that LVLMs have a limited capability for genuine diagram understanding, and their impressive performance in diagram reasoning is an illusion emanating from other confounding factors, such as the background knowledge in the models.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> real_dataset_examples.tex <==


\begin{figure*}
    \begin{tcolorbox}[colback=violet!10, colframe=violet!70!black, title={\large $\question_{\real}(\entity|\kfq,\ncq)$}]
    

    \vspace{1em}
    
    
    \textbf{Question Prompt:} Think step by step before answering the question and show your reasoning. How many entities are in the diagram?
    A) 11  \underline{\textbf{B) 12}} C) 13 D) 10  
    \vspace{1em}

    \centering
    \includegraphics[width=0.4\textwidth]{images/real_diagrams/fw_1831.png}

    \noindent
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4V:} To determine the number of entities in the diagram, I will count each distinct organism or species represented:

        1. Arctic Tern
        2. Polar Bear
        3. Orca
        4. Harp Seal
        5. Harbor Seal
        6. Arctic Cod
        7. Humpback Whale
        8. Capelin
        9. Amphipod
        10. Arctic Char
        11. Copepod
        12. Phytoplankton
        
        There are a total of 12 entities in the diagram.
        
        B) 12
    \end{tcolorbox}

    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4o:} To determine the number of entities in the diagram, we need to count each unique organism or entity represented. Let's list them out:

        1. Arctic Tern
        2. Polar Bear
        3. Orca
        4. Harp Seal
        5. Harbor Seal
        6. Arctic Cod
        7. Humpback Whale
        8. Capelin
        9. Arctic Char
        10. Amphipod
        11. Copepod
        12. Phytoplankton
        
        There are 12 unique entities in the diagram.
        
        Therefore, the correct answer is:
        B) 12
    \end{tcolorbox}
    
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{Gemini 1.5 Pro:} Let's count the entities one by one: Arctic Tern, Polar Bear, Orca, Harp Seal, Harbor Seal, Arctic Cod, Capelin, Arctic Char, Amphipod, Copepod, Humpback Whale, Phytoplankton. There are 12 entities in total.
So the answer is B) 12.
    \end{tcolorbox}
\end{tcolorbox}
\caption{A knowledge-free entity question example for a real FoodWeb diagram.}
\label{app:fig:real:entity_abs}
\end{figure*}


\begin{figure*}
    \begin{tcolorbox}[colback=violet!10, colframe=violet!70!black, title={\large $\question_{\real}(\entity|\krq,\nrq)$}]
    

    \vspace{1em}
    
    
    \textbf{Question Prompt:} Think step by step before answering the question and show your reasoning. Which is the producer in the foodweb?
    A) Harbor Seal \underline{\textbf{B) Phytoplankton}} C) Arctic Cod D) Harp Seal  
    \vspace{1em}

    \centering
    \includegraphics[width=0.4\textwidth]{images/real_diagrams/fw_1831.png}

    \noindent
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4V:} In a food web, the producer is typically an organism that can produce its own food through photosynthesis and serves as the base for the food web. Looking at the options provided:

        A) Harbor Seal - This is a consumer, not a producer.
        B) Phytoplankton - These are microscopic organisms that can photosynthesize, making them producers.
        C) Arctic Cod - This is a consumer, as it feeds on other organisms.
        D) Harp Seal - This is also a consumer, not a producer.
        
        Given this information, the correct answer is:
        
        B) Phytoplankton
    \end{tcolorbox}

    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4o:} To determine the producer in the food web, we need to identify the organism that produces its own food through photosynthesis or chemosynthesis, typically at the base of the food web.

        1. **Harbor Seal**: This is a consumer, as it feeds on other organisms.
        2. **Phytoplankton**: These are microscopic plants that produce their own food through photosynthesis and are typically at the base of the food web.
        3. **Arctic Cod**: This is a consumer, as it feeds on other organisms.
        4. **Harp Seal**: This is a consumer, as it feeds on other organisms.
        
        Given this analysis, the producer in the food web is:
        
        B) Phytoplankton
    \end{tcolorbox}
    
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{Gemini 1.5 Pro:} Producers are the base of the food web and are consumed by other organisms. In this image, all organisms ultimately get their energy from the arrows pointing to them from Phytoplankton. B) Phytoplankton.
    \end{tcolorbox}
\end{tcolorbox}
\caption{A knowledge-required entity question example for a real FoodWeb diagram.}
\label{app:fig:real:entity_know}
\end{figure*}





\begin{figure*}
    \begin{tcolorbox}[colback=violet!10, colframe=violet!70!black, title={\large $\question_{\real}(\relation|\kfq,\nrq)$}]
    

    \vspace{1em}
    
    
    \textbf{Question Prompt:} Think step by step before answering the question and show your reasoning. Which entity is not connected to polar bear?
    A) Harbor Seal B) Harp Seal \underline{\textbf{C) Orca}} D) Arctic Cod
    \vspace{1em}

    \centering
    \includegraphics[width=0.4\textwidth]{images/real_diagrams/fw_1831.png}

    \noindent
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4V:} To determine which entity is not connected to the polar bear, let's examine the connections in the diagram:

        - A) Harbor Seal is connected to the polar bear through a direct arrow pointing from the polar bear to the Harbor Seal.
        - B) Harp Seal is also connected to the polar bear through a direct arrow pointing from the polar bear to the Harp Seal.
        - C) Orca is connected to the polar bear through a direct arrow pointing from the Orca to the polar bear.
        - D) Arctic Cod does not have a direct connection to the polar bear in the diagram. There are no arrows between the Arctic Cod and the polar bear.
        
        Therefore, the correct answer is:
        
        D) Arctic Cod
    \end{tcolorbox}

    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4o:} To determine which entity is not connected to the polar bear, we need to trace the arrows leading to and from the polar bear in the diagram.

        1. **Polar Bear**:
        - Connected to **Harbor Seal** (direct arrow).
        - Connected to **Harp Seal** (direct arrow).
        - Connected to **Orca** (direct arrow).
        
        2. **Arctic Cod**:
        - No direct arrow connecting Arctic Cod to Polar Bear.
        
        Therefore, the entity that is not connected to the polar bear is:
        
        D) Arctic Cod
    \end{tcolorbox}
    
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{Gemini 1.5 Pro:} The polar bear is connected to the harp seal and harbor seal. The polar bear is not connected to the orca.
        The answer is: C) Orca.
    \end{tcolorbox}
\end{tcolorbox}
\caption{A knowledge-free relation question example for a real FoodWeb diagram.}
\label{app:fig:real:relation_abs}
\end{figure*}







\begin{figure*}
    \begin{tcolorbox}[colback=violet!10, colframe=violet!70!black, title={\large $\question_{\real}(\relation|\krq,\nrq)$}]
    

    \vspace{1em}
    
    
    \textbf{Question Prompt:} Think step by step before answering the question and show your reasoning. Which is not the prey of Polar Bear?
    A) Harbor Seal \underline{\textbf{B) Orca}} C) Arctic Cod D) Harp Seal
    \vspace{1em}

    \centering
    \includegraphics[width=0.4\textwidth]{images/real_diagrams/fw_1831.png}

    \noindent
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4V:} B) Orca
    \end{tcolorbox}

    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{GPT-4o:} To determine which is not the prey of the Polar Bear, we need to follow the arrows pointing towards the Polar Bear in the diagram.

        1. The Polar Bear has arrows pointing from:
        - Harbor Seal
        - Harp Seal
        - Orca
        
        2. There is no arrow pointing from Arctic Cod to the Polar Bear.
        
        Therefore, the correct answer is:
        
        B) Orca
    \end{tcolorbox}
    
    \begin{tcolorbox}[colback=gray!10, colframe=gray!80]
        \textbf{Gemini 1.5 Pro:} The arrows in the diagram point from prey to predator. For example, an arrow from "Harp Seal" to "Polar Bear" means that Polar Bears eat Harp Seals.

        - There is an arrow from "Harbor Seal" to "Polar Bear".
        - There is an arrow from "Harp Seal" to "Polar Bear".
        - There is an arrow from "Arctic Cod" to "Harp Seal", and an arrow from "Harp Seal" to "Polar Bear". Therefore, Polar Bears eat Arctic Cod.
        - There is no arrow from "Orca" to "Polar Bear".
        
        Thus, Orca is not a prey of Polar Bear.
        
        **B) Orca**
    \end{tcolorbox}
\end{tcolorbox}
\caption{A knowledge-required entity question example for a real FoodWeb diagram.}
\label{app:fig:real:relation_know}
\end{figure*}






    

    
    



        

        
        

        
        
        
        
    

